Decorrelating ReSTIR Samplers via MCMC Mutations

Monte Carlo rendering algorithms often utilize correlations between pixels to improve efficiency and enhance image quality. For real-time applications in particular, repeated reservoir resampling offers a powerful framework to reuse samples both spatially in an image and temporally across multiple frames. While such techniques achieve equal-error up to 100 times faster for real-time direct lighting and global illumination, they are still far from optimal. For instance, unchecked spatiotemporal resampling often introduces noticeable correlation artifacts, while reservoirs holding more than one sample suffer from impoverishment in the form of duplicate samples. We demonstrate how interleaving Markov Chain Monte Carlo (MCMC) mutations with reservoir resampling helps alleviate these issues, especially in scenes with glossy materials and difficult-to-sample lighting. Moreover, our approach does not introduce any bias, and in practice we find considerable improvement in image quality with just a single mutation per reservoir sample in each frame.

==> Sections/A1_wy_proof.tex <==
\section{Unbiased Contribution Weights and Elimination of Startup Bias}
\label{app:UnbiasedContributionWeights}

Below, we derive unbiased contribution weights for Metropolis-Hastings mutated samples to allow resampled importance sampling with mutations.

We start with sample $X$ and its unbiased contribution weight $W_X$, i.e., for any integrable function $f$, $f(X) W_X$ is an unbiased estimate for the integral of $f$ over the support of $X$. We mutate $X$ into $Y$ via a Metropolis-Hastings mutation with target function $\phat$, and derive weight $W_Y$ such that $f(Y) W_Y$ remains an unbiased estimate for the integral of $f$ over the support of $Y$, making $W_Y$ an unbiased contribution weight and allowing RIS with $Y$. We assume that the support of $X$ exactly covers the support of $\phat$, although it need not be distributed proportionally to $\phat$. We also assume that the mutations retain the full support, i.e., $\supp Y = \supp \phat$.

We first mutate $X$ into a candidate $Z$, distributed proportionally to PDF $q(X \to \cdot)$. We assume that every possible mutation can be reversed (see \emph{detailed balance}, e.g., Veach eq.11.3); $q(x \to z) = 0$ if and only if $q(z \to x) = 0$.

The mutation from $x$ to $z$ is accepted with probability
\begin{equation}
    a(x \to z) = \min\left(1, \frac{\phat(z) q(z \to x)}{\phat(x) q(x \to z)} \right).
\end{equation}
For ease of mathematical manipulation, we also define $a(x \to z) = 0$ if $\phat(x) = 0$ or $q(x \to z) = 0$. This does not modify the transition probabilities: if $\phat(x) = 0$, $x$ is outside $\supp \phat = \supp X$ and is never realized; if $q(x \to z) = 0$, the PDF of realizing $z$ from $x$ is zero.
%
If the mutation from $X$ to the candidate $Z$ is accepted, we set the mutation result $Y = Z$; otherwise we set $Y = X$.

We now want to know a weight $W_Y$ for $Y$ such that 
\begin{equation}
    \E\left[f(Y) W_Y\right] = \int_{\supp Y} f(y) \d{y}
\end{equation}
for all integrable $f$; this $W_Y$ enables using $Y$ with GRIS. We then parametrize $W_Y = g(X \to Y) W_X$ with an unknown two-parameter function $g$, and solve for $g$. The solution is $g(X \to Y) = \phat(X) / \phat(Y)$, which we derive in the following.

\Markus{simplify the derivation}

\subsection{Derivation}

By substitution, we derive
\begin{equation}
    \E\left[f(Y) W_Y\right] = \E\left[f(Y) g(X \to Y) W_X\right],
\end{equation}
which we split by the acceptance condition into
\begin{align}
    = & \E\left[a(X \to Z) f(Z) g(X \to Z) W_X \right. \\
    & \left. + (1 - a(X \to Z)) f(X) g(X \to X) W_X \right].
\end{align}
We then write the expectation over the candidate $Z$ as an integral and reach
\begin{multline}
    %= & \E[W_X \int_{\supp Y} q(X \to z) \left( a(X \to z) f(z) g(X \to z) + \right..% \\
    = \E\left[W_X \int_{\supp Z} q(X \to z) a(X \to z) f(z) g(X \to z) \right. \\
    \left. + q(X \to z) (1 - a(X \to z)) f(X) g(X \to X) \d{z} \right] ,
\end{multline}
where the support of $Z$ is $\supp q(X \to \cdot)$, which depends on $X$. We denote this by $\supp Z(X)$.
The integral in the right-hand-side of $W_X$ is simply a function of $X$. Since $W_X$ is an unbiased contribution weight, we can rewrite this as
\begin{multline}
    = \int_{\supp X} \int_{\supp Z(x)} q(x \to z) a(x \to z) f(z) g(x \to z) \\
        + q(x \to z) (1 - a(x \to z)) f(x) g(x \to x) \d{z} \d{x} .
\end{multline}
We split this integral into three terms:
\begin{align}
    (A) & = \int_{\supp X} \int_{\supp Z(x)} q(x \to z) a(x \to z) f(z) g(x \to z) \d{z}\d{x},\\
    (B) & = \int_{\supp X} \int_{\supp Z(x)} q(x \to z) f(x) g(x \to x) \d{z} \d{x} , \text{\quad and} \notag \\
    (C) & = -\int_{\supp X} \int_{\supp Z(x)} q(x \to z) a(x \to z) f(x) g(x \to x) \d{z} \d{x} , \notag
\end{align}
and manipulate them individually.
%
First, 
\begin{align}
(B) = \int_{\supp X} f(x) g(x \to x) \int_{\supp Z(x)} q(x \to z) \d{z} \d{x} ,
\end{align}
where the integral of $q$ is 1 since it is a PDF in $\supp Z(x)$. To further simplify, we constrain $g$ by assuming $g(x \to x) = 1$; this yields
\begin{align}
(B) = \int_{\supp X} f(x) \d{x} .
\end{align}
Since we assume $\supp X = \supp Y$, this is the result we want; we then find $g$ such the sum of (A) and (C) always equals zero.

From the definition of $a$, we derive the detailed balance condition,
\begin{equation}
    \phat(x) q(x \to z) a(x \to z) = \phat(z) q(z \to x) a(z \to x) .
\end{equation}
Since the outer integral in (A) is over $\supp X = \supp \phat$, all $x$ fulfill $\phat(x) > 0$, and we can rewrite (A) as
\begin{align}
    \int_{\supp X} \int_{\supp Z(x)} q(z \to x) a(z \to x) f(z) \frac{\phat(z)}{\phat(x)} g(x \to z) \d{z}\d{x}.
\end{align}
Next, we extend the integrals into the full domain $\Omega$ by indicator functions; for brevity, we type $\ind_X$ instead of $\ind_{\supp X}$ and similarly for $Z(x)$. We reach
\begin{align}
    \int_{\Omega} \int_{\Omega} \ind_{X}(x) \ind_{Z(x)}(z) q(z \to x) a(z \to x) f(z) \frac{\phat(z)}{\phat(x)} g(x \to z) \d{z}\d{x}.
\end{align}
We then rename the integration variables by $x' = z$ and $z' = x$ and swap the integration order, yielding the following expression for (A):
\begin{align}
    \int_{\Omega} \int_{\Omega} \ind_{X}(z') \ind_{Z(z')}(x') q(x' \to z') a(x' \to z') f(x') \frac{\phat(x')}{\phat(z')} g(z' \to x') \d{z'} \d{x'}.
\end{align}

We then take (C), substitute the constraint $g(x \to x) = 1$ and rewrite it with indicator functions:
\begin{align}
    (C) & = -\int_{\Omega} \int_{\Omega} \ind_X(x) \ind_{Z(x)}(z) q(x \to z) a(x \to z) f(x) \d{z} \d{x} . \notag
\end{align}
We can now write (A) + (C) as
\begin{multline}
    \label{eq:appendix-a-plus-c}
    \int_{\Omega} \int_{\Omega} 
        q(x \to z) a(x \to z) f(x) \\
    \cdot \left( \ind_X(z) \ind_{Z(z)}(x) \frac{\phat(x)}{\phat(z)} g(z \to x) - \ind_X(x) \ind_{Z(x)}(z) \right) \d{z} \d{x} ,
\end{multline}
which we want to be zero.
%For the integrand to be non-zero, we would at least need to have $q(x \to z) > 0$ and $a(x \to z) > 0$. The first condition is equivalent with $z \in \supp Z(x)$, i.e., $\ind_{Z(x)}(z) = 1$. We assume $q(x \to z) > 0$ implies $q(z \to x) > 0$, which implies also $\ind_{Z(z)}(x) = 1$. The latter condition, $a(x \to z) > 0$, implies $\phat(x)$ and $\phat(z)$ are positive, i.e., $\ind_X(x) = \ind_X(z) = 1$. Were the integrand to be non-zero, we should thus additionally have
%\begin{equation}
    %\frac{\phat(x)}{\phat(z)} g(z \to x) - 1 \ne 0,
%\end{equation}
%which we can prevent by choosing $g(z \to x) = \phat(z) / \phat(x)$, yielding
%\begin{equation}
%    W_Y = \frac{\phat(X)}{\phat(Y)} W_X .
%\end{equation}
For the integrand to be non-zero, we would at least need to have $q(x \to z) > 0$ and $a(x \to z) > 0$. The first condition is equivalent with $z \in \supp Z(x)$, i.e., $\ind_{Z(x)}(z) = 1$. We assume $q(x \to z) > 0$ implies $q(z \to x) > 0$, which implies also $\ind_{Z(z)}(x) = 1$. The latter condition, $a(x \to z) > 0$, implies $\phat(x)$ and $\phat(z)$ are positive, i.e., $\ind_X(x) = \ind_X(z) = 1$. Thus, when the first factors in \autoref{eq:appendix-a-plus-c} are non-zero as described above, we enforce the factor in parentheses to be zero by requiring
\begin{equation}
    \frac{\phat(x)}{\phat(z)} g(z \to x) - 1 = 0,
\end{equation}
from which we solve $g(z \to x) = \phat(z) / \phat(x)$, yielding
\begin{equation}
    W_Y = \frac{\phat(X)}{\phat(Y)} W_X .
\end{equation}





==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    # if the dependency isn't one of the files that this latexmk run will consider, process it
    # without this test, we would get an infinite loop!
    if (!($root_filename eq $_[0]))
    {   # PLEASE ENABLE ONLY ONE OF THE FOLLOWING
        # DEPENDING ON THE ENGINE YOU'RE USING
    
        # FOR PDFLATEX
        system( "latexmk -pdf \"$_[0]\"" );

        # FOR LATEX+DVIPDF
        # system( "latexmk \"$_[0]\"" );

        # FOR XELATEX
        # system( "latexmk -xelatex \"$_[0]\"" );
        
        # FOR LUALATEX
        # system( "latexmk -lualatex \"$_[0]\"" );
   }
}
